How Do Source-side Monolingual Word Embeddings Impact Neural Machine Translation?

Using pre-trained word embeddings as input layer is a common practice in many natural language processing (NLP) tasks, but it is largely neglected for neural machine translation (NMT). In this paper, we conducted a systematic analysis on the effect of using pre-trained source-side monolingual word embedding in NMT. We compared several strategies, such as fixing or updating the embeddings during NMT training on varying amounts of data, and we also proposed a novel strategy called dual-embedding that blends the fixing and updating strategies. Our results suggest that pre-trained embeddings can be helpful if properly incorporated into NMT, especially when parallel data is limited or additional in-domain monolingual data is readily available.

==> resources/todo.tex <==
\section*{TODO-items For The Project}

\begin{itemize}
\item Do we want to remove "source-side" and/or "monolingual"?: KD - let's decide after we get all results.
\item Do we want to experiment with more than one language, say Arabic and German? It's generally important for an analysis paper to be reproducible and systematic. Also, it's important that we may want some language pairs that share the same alphabet so we can see whether embeddings with the shared subword space is helpful.: KD - sure, more is better. Let's finish adaptation in one language and then expand. 
\item Run the adaptation experiments.: KD - I think we should focus on these experiments first. Can you start dumping the experiment results in the paper?
% \item Do we want to run experiments that compares with previous methods?: KD - What do you have in mind?
\item Do some analysis on the embeddings. e.g.
	\begin{itemize}
		\item qualitatively analysis -- hopefully the Chinese word for "elder sister" and "younger sister" are clustered closer together?: KD - good idea!
		\item quantitative analysis -- how much correction over the pre-trained embedding are we doing? What trend do we observe when looking at word types of different POS-tags? of different frequency?: KD - yes, we can break down BLEU by sentence then do this kind of analysis.
	\end{itemize}
\end{itemize}

